Towards Reliable and Generalizable Differentially Private Machine Learning (Extended Version)

There is a flurry of recent research papers proposing novel differentially private machine learning (DPML) techniques. These papers claim to achieve new state-of-the-art (SoTA) results and offer empirical results as validation. However, there is no consensus on which techniques are most effective or if they genuinely meet their stated claims. Complicating matters, heterogeneity in codebases, datasets, methodologies, and model architectures make direct comparisons of different approaches challenging. In this paper, we conduct a reproducibility and replicability (R+R) experiment on 11 different SoTA DPML techniques from the recent research literature. Results of our investigation are varied: while some methods stand up to scrutiny, others falter when tested outside their initial experimental conditions. We also discuss challenges unique to the reproducibility of DPML, including additional randomness due to DP noise, and how to address them. Finally, we derive insights and best practices to obtain scientifically valid and reliable results.

==> Gap_exps.tex <==
\subsection{Gap between SGD and DP-SGD}

\wbnote{Not sure whether we need this}



==> tables/reproduciability.tex <==
%
\vfill
\begin{table*}[b!]
\caption{Summary of claimed results in their papers. Note that claimed performance is achieved on CIFAR-10 with $\varepsilon=8$ except for Sander et al.~\cite{sander2022tan} using ImageNet and Bu et al.~\cite{bu2022scalable} using the pre-trained model and $\varepsilon=1$. Especially, Klause et al.~\cite{klause2022differentially} claimed to improve performance from 81.25\% to 82.5\%; Bu et al.~\cite{bu2022scalable} claimed to improve performance from 94.8\% to 96.7\% at $\varepsilon = 1$ with pre-trained model and fine-tune on \cifar{}; Sander et al.~\cite{sander2022tan} claimed to improve performance from 30.2\% to 39.2\% on ImageNet by training from scratch while De et al.~\cite{de2022unlocking} claimed to improve performance from 71.7\% to 81.4\%. Tram\`er and Boneh~\cite{tramer2020differentially}  claimed to improve performance from 55.00\% to 69.3\% on \cifar{}. Luo et al. \cite{luo2021scalable} claimed to improve from 70.8\% to 81.57\% with fewer privacy budget. Bu et al. \cite{bu2022automatic} claimed to improve from 98.04\% to 98.15\% on MNIST. Dormann et al. \cite{dormann2021not} claimed to improve from 66.2\% to 70.1\% on \cifar{}. Catten et al. \cite{cattan2022fine} claimed to improve from 94.7\% to 95.0\%.
Tang et al. \cite{tang2023differentially} claimed to improve performance from 60.59\% to 72.32\% on \cifar{}. }
\label{tab:claimed_results}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l  c c c  |c c c c c  |c}
\toprule
Paper & Method(s) & \multicolumn{3}{c}{Generalizability} & \multicolumn{5}{|c|}{Reliability}  & Claimed improvement\\
& &Multiple Settings & Datasets & Multiple $\varepsilon$ & Open source & Account for param. search & Multiple runs & Bigger than STD & Ablation & \\
\midrule

Bu et al.~\cite{bu2022scalable} & Clipping techniques & $\times$ & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ & N/A\footnote{Because it doesnot report STD, we don't know whether it is bigger than STD or not.} & $\times$  & 1.90\% \\
Bu et al. \cite{bu2022automatic} & Clipping techniques & \checkmark & \checkmark & \checkmark & \checkmark & $\times$ & \checkmark& $\times$ & \checkmark & 0.11\% \\
Klause et al.~\cite{klause2022differentially} & Model architecture & $\times$ & \checkmark & $\times$ & $\times$ & $\times$ & $\times$ & N/A & \checkmark & 1.25\% \\
Sander et al.~\cite{sander2022tan} & Model architecture & $\times$ & \checkmark & $\times$ & \checkmark & $\times$ & \checkmark & \checkmark & \checkmark & 9.00\% \\
Dormann et al. \cite{dormann2021not} & Hyperparameter tuning & $\times$ & \checkmark & $\times$ & \checkmark & $\times$ & \checkmark& \checkmark & \checkmark & 3.90\% \\
De et al.~\cite{de2022unlocking} & Data augmentations and etc. & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 9.70\% \\

Tram\`er and Boneh~\cite{tramer2020differentially}  & Feature selection & $\times$ & \checkmark & \checkmark & \checkmark & $\times$& \checkmark & \checkmark & \checkmark & 14.30\% \\

Cattan et al. \cite{cattan2022fine} & Finetuning technique & N/A  & $\times$ & \checkmark & $\times$ & $\times$ & $\times$ & N/A & $\times$ & 0.3\% \\

Luo et al. \cite{luo2021scalable} & Finetuning technique & N/A  & \checkmark & \checkmark & $\times$ & $\times$ & $\times$ & N/A & \checkmark & 10.77\% \\

Tang et al. \cite{tang2023differentially} & Finetuning technique & N/A  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 11.73\% \\

\bottomrule
\end{tabular}%
}
\end{table*}
%
\vfill
